Domain Knowledge Discovery Guided by Software Trace Links

Software-intensive projects are specified and modeled using domain terminology. Knowledge of the domain terminology is necessary for performing many Software Engineering tasks such as impact analysis, compliance verification, and safety certification. However, discovering domain terminology and reasoning about their interrelationships for highly technical software and system engineering domains is a complex task which requires significant domain expertise and human effort. In this paper, we present a novel approach for leveraging trace links in software intensive systems to guide the process of mining facts that contain domain knowledge. The trace links which drive our mining process, define relationships between artifacts such as regulations and requirements and enable a guided search through high-yield combinations of domain terms. Our proof-of-concept evaluation shows that our approach aids in the discovery of domain facts even in highly complex technical domains. These domain facts can provide support for a variety of Software Engineering activities. As a use case, we demonstrate how the mined facts can facilitate the task of project Q&A.

==> Ontology-Introduction.tex <==
\section{Introduction}
\label{sec:Introduction}
Software and systems engineering projects are situated across a diverse set of domains including transportation, communication and control, medical devices, finance, electronic health care, and aeronautics. Each of these domains is characterized by its own concepts and terminology.  As a result, project stakeholders, such as requirements engineers, architects, developers, and safety analysts, use the domain terminology to specify requirements, define components, label model elements, and to provide meaningful class, method, and variable names in the source code \cite{DBLP:books/daglib/p/LuciaMOP12}. Defining the meanings of terms, and explicitly capturing relationships between them, facilitates a host of software and requirements engineering activities. For example, in a \emph{Question-and-Answer} tool, a user might request ``all requirements related to security of \emph{medical devices}'' \cite{DBLP:conf/re/PruskiLAOARC14, DBLP:journals/computer/Cleland-HuangBCSR07}. This question can only be fully answered if it is understood that devices such as \emph{infusion pumps} and \emph{heart rate monitors} are types of medical devices. Such relations between concepts can be captured in an \emph{ontology}. An ontology provides formal definitions of concepts, identifies synonyms, expands acronyms, and captures relationships such as \emph{is-a} and \emph{part-of}. A \emph{domain} ontology, as its name implies, captures the specific terminology and meanings that are common to a specific domain \cite{DBLP:journals/semweb/Guizzardi10}. 

In current practice, very few projects are supported by ontologies, but many include a basic project glossary defining terms and acronyms \cite{DBLP:conf/esem/AroraSBZ14, DBLP:conf/serp/ZouSC08}.  Unfortunately, while glossaries tend to provide definitions of terms, especially acronyms, they typically fail to capture relationships between domain concepts and therefore fall short of providing the kind of knowledge needed to accurately automate many software engineering analysis tasks. For example, an automated traceability tool is tasked with inferring the similarity between different artifacts and constructing trace links accordingly even when artifacts are specified using different terminology. In many cases, trace links need to be created between artifacts of different types, such as between requirements and design, and this typically means that they will be specified using different terminology at disparate levels of abstraction \cite{DBLP:conf/re/0004CB13}. Similarly,  ambiguity detection tools must analyze multiple requirements in order to identify potential conflicts and ambiguities \cite{DBLP:journals/re/YangRGWN11}, and design satisfaction tools must compare the extent to which topics are specified in requirements versus their coverage in the design \cite{DBLP:journals/ese/HolbrookHDL13}.

Ontologies can be time-consuming to construct \cite{DBLP:journals/kbs/GacituaSR08, DBLP:conf/awic/OhtaKM11, DBLP:conf/skg/LiuXL11, Cerquitelli:2011:SOC:2441488.2441489} and are therefore typically unavailable for the diverse set of technical domains in which systems engineering projects reside. Many software-intensive products live on for decades, evolving continually as features are added and new products released. Despite the effort required to create them, domain ontologies are likely to provide significant long-term return on investment \cite{DBLP:conf/skg/LiuXL11} as they can be reused across multiple projects in a domain, and progressively evolved as new concepts are introduced.

In this paper we present a novel solution for building ontology within the context of software and systems engineering projects. While numerous researchers have proposed and developed techniques for building ontology, our approach is unique in the way that it leverages traceability data to supervise the process. Software traceability is defined as ``the ability to interrelate any uniquely identifiable software engineering artifact to any other, maintain required links over time, and use the resulting network to answer questions of both the software product and its development process'' \cite{DBLP:conf/icse/Cleland-HuangGHMZ14}. Developers of many software systems, especially those in the safety-critical domain, are required by certification processes to create and maintain an extensive network of traceability links. Each link is defined in terms of a {\bf source} artifact and a {\bf target} artifact, associated by a {\bf semantically-typed relationship}. For example, a requirement might be traced to a regulatory code with a \emph{complies to} link, or an element of the design (such as a class in a UML diagram) might be traced to a mitigating requirement with a \emph{mitigates} link. Such trace links have been created and scrutinized by domain experts and can serve as an effective, and previously unexplored, resource for ontology building.

Our approach utilizes several different techniques, all ultimately driven-by, or supervised-by the traceability data. Natural language processing is used to extract domain terms and phrases, data mining and pattern matching to identify relations that are explicitly defined in domain documents, and finally topic modeling and association rule mining to discover additional associations. We use these techniques to extract candidate facts from domain documents and from software and systems artifacts such as requirements and design specifications, and then leverage existing trace links to guide the ontology construction process. Our approach is depicted in Figure \ref{fig:Overview}. 

\begin{figure}[!t]	
	\centering
	\includegraphics[width=.6\textwidth]{Overview4.pdf}	
	\vspace{-4pt}
	\caption{ An Overview of our Ontology Extraction}
	\label{fig:Overview}
\end{figure}

The remainder of the paper is laid out as follows. Section \ref{sec:DomainConcepts} introduces the two domains of our study and describes their characteristics. Section \ref{sec:IdentifyCandidateFact} presents the details of four different techniques for mining ontology facts from domain documents and software artifacts.  Sections \ref{sec:Links} then describes how we leverage traceability data to supervise the ontology learning process and reports results from applying it across the two domains in Section \ref{sec:Evaluation}. Finally, Sections \ref{sec:Threats} to \ref{sec:Conclusion} discuss threats to validity, related work, and then provide a summary of our findings.

\begin{table}[!t]
	\caption{Systems Engineering Domains}
	\label{tab:Domains}
	\centering
	\small\addtolength{\tabcolsep}{-3.5pt}
	%\tiny 
	\begin{tabular}{|L{1.2cm}|L{2cm}|L{2cm}|L{2.5cm}|}
		\hline
		\textbf{Domain}&\textbf{Description}&\textbf{Domain Documents}&\textbf{Software Artifacts} \\ \hline
			Electronic Health Records (EHR)& Systems for managing digital healthcare records.&100 files \newline(79 MBytes) describing electronic health records&\textbf{1064} CCHIT regulatory guidelines\newline \textbf{116} WorldVista Requirements\newline {\bf 589 Trace links} \\ \hline
		Medical Infusion Pumps (MIP)&Systems for controlling the delivery of fluids to a patient (e.g. insulin pump).&100 files \newline(83 MBytes) describing features and process of MIP&{\bf 126} Requirements \newline {\bf 22} Component Descriptions \newline {\bf 131 Trace links}\\ \hline		
	\end{tabular}
\end{table}

==> Ontology-LeveragingLinks.tex <==
\section{Validating Candidate Facts}
\label{sec:Links}
In the previous section we presented four techniques for generating candidate facts. In this section we describe our novel traceability driven approach for transforming these candidate facts into a validated ontology. Our approach leverages the project's traceability data to incrementally build the ontology. 
Consider the following trace link between a requirement and design element:\vspace{6pt}\\
\noindent
\begin{tabular}{L{3.6cm}|p{8.5cm}}
	
	\textbf{Artifact }&\textbf{Artifact Text}\\ \hline
	{\bf Design (D1)} (Source) &The PCA pump shall have a start button.\\ \hline
	{\bf Requirement (R1)} (Target) &The control panel combines a touch panel with a speaker by which a clinician can enter and confirm configuration and see and hear alarms and warnings.\\ 	
\end{tabular} \\

Even though the design artifact and the requirement exhibit almost no shared terms, the presence of a validated trace link tells us that they must somehow be related. At least one element (noun, noun phrase or verb) in the requirement must be related to at least one element in the design. Our approach leverages this traceability data to guide the validation of candidate facts.  Given a specific trace link, we retrieve the set of relevant facts from the existing ontology as well as from the pool of candidate facts which could explain the link. The retrieved candidate facts are then ranked heuristically. In future work we plan to build training sets of facts and use machine learning to dynamically discover the best way to combine evidence from our four fact mining techniques.

\subsection{Ranking Heuristics}
\label{subsec:RankFacts}
Each trace link can yield a large number of term combinations, referred to as candidate facts (CFs). For \emph{proof-of-concept} purposes we developed the following heuristics which utilize the four techiniques described earlier to filter and rank the CFs. Our heuristics are based on observations about the individual and combined accuracy of the four techniques.  We assume the terminology that $Ev_{TX}$ means that technique $TX$ supports the CF. Furthermore, $DS$ is domain specificity from Equation \ref{eq:ontology_DomainSpecificity}, $S_{term}$ and $T_{term}$ represent the set of words in source term and target artifacts respectively.  \vspace{6pt}\\
\noindent 1. Remove the $cf$ if $\neg Ev_{TM} \lor \neg Ev_{SEM}$.\\
\noindent 2. Assign confidence scores $Conf$ (See Table \ref{tab:Heuristics})\\
\noindent 3. Rank all $CF$s by $Conf$ score. In case of a tie, rank by the product of $Ev_{TM}$ and $Ev_{SEM}$ measures. For further tie, rank by the $Ev_{ARM}$ measure.\\
\noindent 4. Accept top $N$ candidate facts or all facts over a specified confidence score. 

\begin{table}[!h]
  \caption{Heuristics for Computing Confidence Scores}
  \label{tab:Heuristics}
  \vspace{-5pt}
  \centering
  \includegraphics[width=0.65\linewidth]{Heuristics.pdf}
\end{table}
\vspace{-5pt}


Given the trace link shown earlier between Requirement $R1$ and Design artifact $D1$ we ranked all of the generated candidate facts using these heuristics. Our tool generated seven candidate facts depicted in Table \ref{tab:RankedFact}.  Only facts generated using syntactic relatedness include labeled relationships.  In this example, the first candidate fact states that \emph{start button {\bf press of}(Reverse direction) clinician}. Other facts identify unlabeled relationships such as \emph{pca pump} is associated with \emph{control panel}.

\begin{table}[h]
\caption{Generated Candidate Facts }
\centering
\begin{tabular}{|L{1cm}|L{2.5cm}|L{2.5cm}|L{3.2cm}|L{2cm}|}
		\hline
		\textbf{Rank}& \textbf{Source Entity} & \textbf{Target Entity} & \textbf{Suggested Relation} & \textbf{Conf. Score} \\ \hline
		1&start button&clinician& press of $(Reverse)$& 0.9 \\ \hline 
		2&pca pump&touch panel&& 0.6 \\ \hline
		3&pca pump&control panel&& 0.5 \\ \hline 
		4&pca pump&alarm&& 0.5 \\ \hline
		5&pca pump&clinician&& 0.4 \\ \hline
		6&start button&touch panel&& 0.1 \\ \hline
		7&start button&control panel&& 0.1 \\ \hline 
\end{tabular}
\label{tab:RankedFact}
\vspace{-6pt}
\end{table}

\begin{table}[h]
	\caption{Facts accepted by the User}
	
\centering
\begin{tabular}{|L{1cm}|L{2.5cm}|L{2.5cm}|L{3cm}|}
				\hline
				\textbf{Index}& \textbf{Source Entity} & \textbf{Target Entity} & \textbf{Relation} \\ \hline
				1&start button&clinician& is pressed by \\ \hline 
				2&pca pump&touch panel&contains\\ \hline
				3&pca pump&control panel&contains\\ \hline 
				4&start button&touch panel&is located on \\ \hline
				5&start button&control panel&is located on\\ \hline 
			\end{tabular}
			\label{tab:AcceptedFact}	
\end{table}

At this point, the ontology can be generated in a fully automated way by accepting the top N candidate facts for each trace link, or by accepting all facts over a certain confidence score.  Alternately, the ranked facts can be presented to a human analyst to allow them to vet the facts before saving them in the ontology.

\subsection{Adding the Human into the Loop}
Our GUI tool supports the user in the task of vetting and modifying candidate facts. The user may accept or reject the candidate facts and also modify any part of its description. Table \ref{tab:AcceptedFact} shows the final facts accepted and modified by a human user. In this case the user accepted five of the recommended facts, added the missing relations and then saved the validated facts to the ontology. In Figure \ref{fig:ProtegeView} we provide a view of part of the MIP ontology constructed using the Web Ontology Language (OWL)\footnote{https://www.w3.org/TR/owl-features/} following the human vetting process.












==> output.tex <==
\begin{thebibliography}{10}

\bibitem{AS94}
R.~Agrawal and R.~Srikant.
\newblock Fast algorithms for mining association rules.
\newblock In {\em Proc. of the 20th Intn'l Conf. on Very Large Data Bases
  (VLDB'94)}, pages 487--499, Santiago, Chile, September 1994.

\bibitem{DBLP:conf/esem/AroraSBZ14}
C.~Arora, M.~Sabetzadeh, L.~C. Briand, and F.~Zimmer.
\newblock Improving requirements glossary construction via clustering: approach
  and industrial case studies.
\newblock In {\em 2014 {ACM-IEEE} Int's Symp. Empirical Software Engineering
  and Measurement, {ESEM}, Torino, Italy, 2014}, 2014.

\bibitem{DBLP:journals/ao/Aussenac-GillesS05}
N.~Aussenac{-}Gilles and D.~Soergel.
\newblock Text analysis for ontology and terminology engineering.
\newblock {\em Applied Ontology}, 1(1):35--46, 2005.

\bibitem{blei2003latent}
D.~M. Blei, A.~Y. Ng, and M.~I. Jordan.
\newblock Latent dirichlet allocation.
\newblock {\em the Journal of machine Learning research}, 3:993--1022, 2003.

\bibitem{OntolgyAsReProduct}
K.~K. Breitman and J.~C.~S. do~Prado~Leite.
\newblock Ontology as a requirements engineering product.
\newblock In {\em Requirements Engineering Conference, 2003. Proceedings. 11th
  IEEE International}, pages 309--319, Sept 2003.

\bibitem{CCHIT}
{CCHIT Guidelines}.
\newblock {Certification Commission for Healthcare Information
  Technology},guidelines for electronic healthcare records, 2010.
\newblock Previously available at {http://cchit.org}.

\bibitem{Curran07minimisingsemantic}
J.~R. Curran, T.~Murphy, and B.~Scholz.
\newblock Minimising semantic drift with mutual exclusion bootstrapping.
\newblock In {\em Conf. of the Pacific Association for Computational
  Linguistics}, pages 172--180, 2007.

\bibitem{dobson2006revisiting}
G.~Dobson and P.~Sawyer.
\newblock Revisiting ontology-based requirements engineering in the age of the
  semantic web.
\newblock In {\em Proceedings of the International Seminar on Dependable
  Requirements Engineering of Computerised Systems at NPPs}, pages 27--29,
  2006.

\bibitem{DBLP:conf/ACISicis/GacituaS08}
R.~Gacitua and P.~Sawyer.
\newblock Ensemble methods for ontology learning - an empirical experiment to
  evaluate combinations of concept acquisition techniques.
\newblock In {\em 7th {IEEE/ACIS} International Conference on Computer and
  Information Science, {IEEE/ACIS} {ICIS} 2008, 14-16 May 2008, Portland,
  Oregon, {USA}}, pages 328--333, 2008.

\bibitem{DBLP:journals/kbs/GacituaSR08}
R.~Gacitua, P.~Sawyer, and P.~Rayson.
\newblock A flexible framework to experiment with ontology learning techniques.
\newblock {\em Knowl.-Based Syst.}, 21(3):192--199, 2008.

\bibitem{DBLP:conf/re/0004CB13}
J.~Guo, J.~Cleland{-}Huang, and B.~Berenbach.
\newblock Foundations for an expert system in domain-specific traceability.
\newblock In {\em 21st {IEEE} International Requirements Engineering
  Conference, {RE} 2013, Rio de Janeiro-RJ, Brazil, July 15-19, 2013}, pages
  42--51, 2013.

\bibitem{EMSEJin}
J.~Guo, M.~Gibiec, and J.~Cleland-Huang.
\newblock Tackling the term-mismatch problem in automated trace retrieval.
\newblock {\em Empirical Software Engineering}, 22(3):1103--1142, Jun 2017.

\bibitem{DBLP:conf/icse/HatcliffWKCJ14}
J.~Hatcliff, A.~Wassyng, T.~Kelly, C.~Comar, and P.~L. Jones.
\newblock Certifiably safe software-dependent systems: challenges and
  directions.
\newblock In {\em Proceedings of the on Future of Software Engineering, {FOSE}
  2014, Hyderabad, India, May 31 - June 7, 2014}, pages 182--200, 2014.

\bibitem{Hearst:1992:AAH:992133.992154}
M.~A. Hearst.
\newblock Automatic acquisition of hyponyms from large text corpora.
\newblock In {\em Proceedings of the 14th Conference on Computational
  Linguistics - Volume 2}, COLING '92, pages 539--545, Stroudsburg, PA, USA,
  1992. Association for Computational Linguistics.

\bibitem{DBLP:conf/swb/HeymansMAMSPMFKKSSFHWK08}
S.~Heymans, L.~Ma, D.~Anicic, Z.~Ma, N.~Steinmetz, Y.~Pan, J.~Mei, A.~Fokoue,
  A.~Kalyanpur, A.~Kershenbaum, E.~Schonberg, K.~Srinivas, C.~Feier, G.~Hench,
  B.~Wetzstein, and U.~Keller.
\newblock Ontology reasoning with large data repositories.
\newblock In {\em Ontology Management, Semantic Web, Semantic Web Services, and
  Business Applications}, pages 89--128. 2008.

\bibitem{DBLP:journals/ese/HolbrookHDL13}
E.~A. Holbrook, J.~H. Hayes, A.~Dekhtyar, and W.~Li.
\newblock A study of methods for textual satisfaction assessment.
\newblock {\em Empirical Software Engineering}, 18(1):139--176, 2013.

\bibitem{kof2005appfication}
L.~Kof.
\newblock An appfication of natural language processing to domain modeliing:
  Two case studies.
\newblock {\em International Journal of Computer Systems Science \&
  Engineering}, 20(1):37--51, 2005.

\bibitem{lin1998information}
D.~Lin.
\newblock An information-theoretic definition of similarity.
\newblock In {\em ICML}, volume~98, pages 296--304, 1998.

\bibitem{DBLP:books/daglib/p/LuciaMOP12}
A.~D. Lucia, A.~Marcus, R.~Oliveto, and D.~Poshyvanyk.
\newblock Information retrieval methods for automated traceability recovery.
\newblock In {\em Software and Systems Traceability.}, pages 71--98. 2012.

\bibitem{miller1995wordnet}
G.~A. Miller.
\newblock Wordnet: a lexical database for english.
\newblock {\em Communications of the ACM}, 38(11):39--41, 1995.

\bibitem{omoronyia2010domain}
I.~Omoronyia, G.~Sindre, T.~St{\aa}lhane, S.~Biffl, T.~Moser, and W.~Sunindyo.
\newblock A domain ontology building process for guiding requirements
  elicitation.
\newblock In {\em Requirements Engineering: Foundation for Software Quality},
  pages 188--202. Springer, 2010.

\bibitem{DBLP:conf/re/PruskiLAOARC14}
P.~Pruski, S.~Lohar, R.~Aquanette, G.~Ott, S.~Amornborvornwong, A.~Rasin, and
  J.~Cleland{-}Huang.
\newblock Tiqi: Towards natural language trace queries.
\newblock In {\em {IEEE} Int'l Requirements Engineering Conference, {RE}
  Karlskrona, Sweden, 2014}, pages 123--132, 2014.

\bibitem{MIPRequirements}
B.~{R. Larson}.
\newblock Santos technical report: 2012-01-24 integrated clinical environment
  patient-controlled analgesia infusion pump system requirements.
\newblock DRAFT 0.9.3, 2012-01-25, Kansas State University.

\bibitem{DBLP:conf/nldb/Ruiz-CasadoAC05}
M.~Ruiz{-}Casado, E.~Alfonseca, and P.~Castells.
\newblock Automatic extraction of semantic relationships for wordnet by means
  of pattern learning from wikipedia.
\newblock In {\em Conf. on Applications of Natural Language to Information
  Systems, {NLDB} 2005, Alicante, Spain}, pages 67--79, 2005.

\bibitem{DBLP:journals/dke/Ruiz-CasadoAC07}
M.~Ruiz{-}Casado, E.~Alfonseca, and P.~Castells.
\newblock Automatising the learning of lexical patterns: An application to the
  enrichment of wordnet by extracting semantic relationships from wikipedia.
\newblock {\em Data Knowl. Eng.}, 61(3):484--499, 2007.

\bibitem{DBLP:conf/nips/SnowJN04}
R.~Snow, D.~Jurafsky, and A.~Y. Ng.
\newblock Learning syntactic patterns for automatic hypernym discovery.
\newblock In {\em Advances in Neural Information Processing Systems 17 [Neural
  Information Processing Systems, {NIPS} 2004, December 13-18, 2004, Vancouver,
  British Columbia, Canada]}, pages 1297--1304, 2004.

\bibitem{wang2012relation}
C.~Wang, A.~Kalyanpur, J.~Fan, B.~K. Boguraev, and D.~Gondek.
\newblock Relation extraction and scoring in deepqa.
\newblock {\em IBM Journal of Research and Development}, 56(3.4):9--1, 2012.

\bibitem{WVista}
{World Vista}.
\newblock {Department of Veterans Affairs Office of Enterprise Development}
  vista-healthvet monograph.

\bibitem{Wu:2012:PPT:2213836.2213891}
W.~Wu, H.~Li, H.~Wang, and K.~Q. Zhu.
\newblock Probase: A probabilistic taxonomy for text understanding.
\newblock In {\em Int'l Conf. on Management of Data}, SIGMOD '12, pages
  481--492, New York, NY, USA, 2012. ACM.

\bibitem{DBLP:journals/re/YangRGWN11}
H.~Yang, A.~N.~D. Roeck, V.~Gervasi, A.~Willis, and B.~Nuseibeh.
\newblock Analysing anaphoric ambiguity in natural language requirements.
\newblock {\em Requir. Eng.}, 16(3):163--189, 2011.

\bibitem{DBLP:conf/serp/ZouSC08}
X.~Zou, R.~Settimi, and J.~Cleland{-}Huang.
\newblock Evaluating the use of project glossaries in automated trace
  retrieval.
\newblock In {\em Software Engineering Research {\&} Practice, {SERP} 2008, Las
  Vegas Nevada, USA}, pages 157--163, 2008.

\end{thebibliography}

